CoRD: Converged RDMA Dataplane for High-Performance Clouds

High-performance networking is often characterized by kernel bypass which is considered mandatory in high-performance parallel and distributed applications. But kernel bypass comes at a price because it breaks the traditional OS architecture, requiring applications to use special APIs and limiting the OS control over existing network connections. We make the case, that kernel bypass is not mandatory. Rather, high-performance networking relies on multiple performance-improving techniques, with kernel bypass being the least effective. CoRD removes kernel bypass from RDMA networks, enabling efficient OS-level control over RDMA dataplane.

==> availability.tex <==
%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.

==> related.tex <==
\section{Related Work}


% \cite{freeflow} and \cite{srdma} add additional hop at the high-performance
% network datapath either as a dedicated CPU core or as a bump-in-a-wire SmartNIC.
% %
% We are driven by the same motivation as other approaches, but we believe the
% same result can be achieved in a much simpler classical OS architecture with the
% same or better performance.


% Kernel-bypass approaches attempt to offload the CPU, sometimes,
% entirely~\cite{joelniderLastCPU2021, brunellaHyperionUnifiedZeroCPU2022}.
% %
% Nevertheless, virtually never want these approaches abandon the CPUs completely,
% instead the goal is to save the CPU cycles for \enquote{other} applications.
% %
% In this context, our goal is to complement kernel bypass, by providing a way for
% the \enquote{other} applications use high-performance networking.

% Arrakis~\cite{arrakis} introduced \emph{filter} functions to intercept data
% plane operations, but acknowledged that hardware-level filters are inflexible.
% %
% Instead, Arrakis relied on emulation of these capabilities on a dedicated CPU
% core.

% Intel proposed DSA~\cite{dsa}, an ibverbs-like hardware interface allowing
% more flexible and more dynamic resource management than SR/IOV~\cite{pcie5}.
% %
% As part of oneAPI~\cite{intelOneAPISpecification2rev1}, DSA enables high
% performance virtualization and intercommunication for wide range of devices.

